THE COLOSSEUM: A Benchmark for Evaluating Generalization for Robotic Manipulation

To realize effective large-scale, real-world robotic applications, we must evaluate how well our robot policies adapt to changes in environmental conditions. Unfortunately, a majority of studies evaluate robot performance in environments closely resembling or even identical to the training setup. We present THE COLOSSEUM, a novel simulation benchmark, with 20 diverse manipulation tasks, that enables systematical evaluation of models across 14 axes of environmental perturbations. These perturbations include changes in color, texture, and size of objects, table-tops, and backgrounds; we also vary lighting, distractors, physical properties perturbations and camera pose. Using THE COLOSSEUM, we compare 5 state-of-the-art manipulation models to reveal that their success rate degrades between 30-50% across these perturbation factors. When multiple perturbations are applied in unison, the success rate degrades $\geq$75%. We identify that changing the number of distractor objects, target object color, or lighting conditions are the perturbations that reduce model performance the most. To verify the ecological validity of our results, we show that our results in simulation are correlated ($\bar{R}^2 = 0.614$) to similar perturbations in real-world experiments. We open source code for others to use THE COLOSSEUM, and also release code to 3D print the objects used to replicate the real-world perturbations. Ultimately, we hope that THE COLOSSEUM will serve as a benchmark to identify modeling decisions that systematically improve generalization for manipulation. See https://robot-colosseum.github.io/ for more details.

==> sections/06_analysis.tex <==
\section{Analysis}
\label{sec:analysis}


\subsection{Failure Analysis}



\paragraph{Distractor} Distractors on the tabletop affect the model's focus on the target object. We notice that in \texttt{basketball in hoop} task, the model confuses the ball with distractors on the table, leading to task failure.

\paragraph{Manipulation Object Size} In imitation learning models, the robot overfits to the object's size that it directly interacts with. Therefore, when the size of the object decreases, it affects the grasp of the object (\texttt{slide block to target}), and when it increases, we notice that the agent ends up colliding with the object (\texttt{open drawer})

\paragraph{Light color} Light color directly affects the input space of the learning models that learn end-to-end with RGB values as part of the input, therefore, affecting the input-to-action mapping of the model.



==> sections/rebuttal_response.tex <==

\newcommand{\hsnote}[1]{{\color{magenta} [HS: #1] }}
\newcommand{\synote}[1]{{\color{blue} [SY: #1]}}
\newcommand{\axnote}[1]{{\color{orange} [AX: #1]}}
\newcommand{\ac}[1]{{\textbf{AC}}}
\newcommand{\rone}[1]{{\color{blue} R1}}
\newcommand{\rtwo}[1]{{\color{magenta} R2}}
\newcommand{\rthree}[1]{{\color{orange} R3}}
\newcommand{\rfour}[1]{{\color{red} R4}}
\section*{Rebuttal response to all}
We thank the AC (\ac{}[KCuP]) and reviewers (\rone{}[C7Vu], \rtwo{}[kbFJ], \rthree{}[fLen]) for their comprehensive and constructive feedback. We appreciate the unanimous recognition of the importance of \benchname\, especially in addressing often-overlooked issues of model generalization, which is critical for scaling up robot data. We are encouraged by the positive reception and wish to highlight the specific commendations received for our work:
\begin{itemize}
    \item “The reviews for the paper all appreciate the importance of a systematic study in representation learning” (\ac{})
    \item “Provides a valuable contribution toward that goal.”, and “Good coverage of tasks, variations, and representative methods from the literature.” (\rone{})
    \item “Help researchers in this field better evaluate their algorithms under different variations.”, and “making the simulation results more convincing and useful for evaluating different algorithms” (\rtwo{})
    \item “Important area to ablate algorithms yet under-served by existing benchmarks.” (\rthree{})
\end{itemize}
% Summary of major responses and issues raised by the reviews (see individual responses for more detail):

% \textbf{Oversimplification on perturbation factors and motivation for selecting these perturbation factors:} Our selection of perturbation factors is informed by recent, diverse, real-world robotics datasets. We have developed a taxonomy based on the various environmental and object perturbations observed in these large-scale datasets. Additionally, we introduce a real-world ablation study that examines pairs of scenarios.  
% We further introduce a real-world ablation study that analyzes pairs of scenarios. One scenario features a composite of perturbations derived from the COLOSSEUM perturbation factors, while the other encompasses a realistic setting where the same perturbations occur naturally. By assessing the correlation between these scenarios, we justify the simplification of perturbation factors and demonstrate their relevance to real-world scene.

% \textbf{Comparison with other generalization benchmarks:}


% \textbf{ Additional physical property perturbation and baselines:}


\section*{Response to AC and individual reviewers}
We have addressed all queries from the AC and reviewers individually. However, due to some overlapping questions between the AC and reviewers, we have grouped them together for clarity.

[\ac{}] \textbf{Oversimplification of perturbation factors and discussion on compounding effects of different perturbation:} 
We investigate how \benchname\'s perturbations can be grounded in the real-world scenarios.Hence, we introduce an additional real-world ablation study (Section \ref{subsec:real-world-ablation} and Figure \ref{fig:rebuttal}) that analyzes pairs of scenarios with one scenario featuring a composite of perturbations derived from \benchname\ perturbation factors, while the other encompasses a realistic setting where the same perturbations occur naturally. To assess the correlation between these scenarios, we evaluated a policy trained without perturbations on these two sets of scenarios. From the experiment, we observed a strong correlation between systematically compounded perturbations and realistic real-world scenarios in two out of three cases. Therefore, simplifying perturbation factors can be relevance to real-world scenarios. We also included discussion evaluation on \texttt{All Perturbations}, and their compounding effects across tasks in Section \ref{sub:all_perturbation}.

[\ac{}, \rtwo{}] \textbf{Comparison with other generalization benchmarks and discussion with RL generalization benchmarks:} We acknowledge the reviewer's feedback and have expanded the discussion in the related work section, incorporating the citations suggested by the reviewer \rtwo{}. Additionally, we have underscored the uniqueness of our benchmark by curating a comparison table (Table 1) that highlights key distinctions, such as the number of perturbations, tasks, state-of-the-art models evaluated, and real-world applicability. While other benchmarks have their merits, our benchmark is currently the most comprehensive in evaluating the generalization of robot manipulation policies in this field. We recognize the presence of numerous RL generalization benchmarks. However, our benchmark differentiates itself by comprising tasks with higher complexity and longer horizons tasks, unlike those RL generalization benchmarks which are designed primarily for RL policies. However, our benchmarks are not limited to Behavior Cloning (BC) models; \benchname\ can also be used to evaluate other types of robotic manipulation policies. For example, we have included VoxPoser as an additional baseline to demonstrate the versatility of our benchmarks in accommodating various approaches. Furthermore unlike other benchmark, we are also presenting \benchname\ as an open challenge to the community, aiming to enhance decision-making regarding model selection for scaling robot data.

[\ac{}, \rthree{}] \textbf{Physical properties perturbation:} We concur with the reviewer's assertion on the necessity of benchmarking a model's generalization across physical properties. Hence to accommodate for this, we have incorporated mass and friction perturbations in our revised work, and detailed them in Section \ref{subsec:mass}. However, we would like to emphasize that the impact of such perturbations is task-specific. In many quasi-static tasks, changes in physical properties—such as mass, friction, and inertia—do not significantly influence outcomes. Conversely, tasks involving dynamic motion \cite{memmel2023asid}, such as a ball's trajectory after being struck by a hockey stick, are notably affected by these variations. Hence, we implemented mass and friction perturbations only specific tasks from \benchname\'s tasks list. Based on our further evaluation of these perturbations, we found that 2D models fail to adapt to changes in physical properties. In contrast, among 3D-based models, \texttt{RVT} significantly outperforms \texttt{PerAct}, demonstrating greater robustness in keypoint prediction for dynamic tasks with such perturbations.

% \textbf{Comparison with other generalization benchmarks:} We addressed this by curating a comparison table (Table I) highlighting key distinctions, such as the number of variations, tasks, state-of-the-art models evaluated, and real-world applicability. While other benchmarks have their merits, to date, our Colosseum benchmark stands as the most comprehensive in this field. Unlike others, we are also presenting it as an open challenge to the community, aiming to enhance decision-making regarding model selection for scaling robot data.

% \textbf{Physical properties perturbation:} We concur with the AC's assertion on the necessity of benchmarking a model's generalization across physical properties. However, we emphasize that the impact of such perturbations is task-specific. In many quasi-static tasks, changes in physical properties—such as mass, friction, and inertia—do not significantly influence outcomes. Conversely, tasks involving dynamic motion \cite{memmel2023asid}, such as a ball's trajectory after being struck by a hockey stick, are notably affected by these variations. Our benchmarks support a wide range of manipulation policies to enable comprehensive evaluation. Hence to accommodate to this, we have incorporated mass and friction perturbations in our revised work, as detailed in Section \ref{subsec:mass}.

[\rone{}]
\textbf{Analysis on leveraging some amount of variations in training:} We agree with the reviewers that a thorough analysis leveraging perturbation data during training can provide deeper insights into deficiencies in our model. Consequently, we have conducted an ablation study, training with data containing \texttt{All Perturbations} evaluating on the same. The results, discussed in Section \ref{sub:all_perturbation}, indicate an inherent upper bound in performance, even with perturbed data used in training. While we could not isolate the effects of specific perturbations on individual models due to inherent differences in their characteristics. However, our benchmark design can still allow users to systematically evaluate their models by training on specific variations. This approach helps determine which perturbations beneficially or adversely affect their models on an individual basis. 

% \subsection{Reviewer  kbFJ}
% \textbf{Comparison with other generalization benchmarks and discussion with RL generalization benchmarks:} We acknowledge the reviewer's feedback and have expanded the discussion in the related work section, incorporating the citations suggested by the reviewer. Additionally, we have underscored the uniqueness of our benchmark by curating a comparison table (Table I) that highlights key distinctions, such as the number of variations, tasks, state-of-the-art models evaluated, and real-world applicability. While other benchmarks have their merits, our Colosseum benchmark currently stands as the most comprehensive in this field. Our tasks are categorized into different levels of complexity and horizons based on the way-points required to achieve the task, distinguishing our benchmark from those designed primarily for RL policies. However, our benchmarks are not limited to Behavior Cloning (BC) models alone; they can also evaluate other types of robotic manipulation policies. For example, we have included VoxPoser as an additional baseline to demonstrate the versatility of our benchmarks in accommodating various approaches. Furthermore unlike other benchmark, we are also presenting it as an open challenge to the community, aiming to enhance decision-making regarding model selection for scaling robot data.

[\rtwo{}] \textbf{FactorWorld has 19 instead of 11 mentioned in the related work:} In the submitted paper, we have stated that "Factor World [62] and KitchenShift [63] are similar efforts
to THE COLOSSEUM, but have 11 and 7 perturbation types" referring to FactorWorld has 11 perturbation tasks and KitchenShift has 7. However, we rephrase it to be clearer to avoid any confusion. 

[\rtwo{}] \textbf{Rationale for selecting particular variations: }We study recent real-world diverse robot datasets, such as, Open-X\cite{open_x_embodiment_rt_x_2023}, DROID\cite{khazatsky2024droid}, Ego4D\cite{Ego4D2022CVPR}, etc., and conclude that our identified factors indeed exist in these datasets. While these factors do not cover the exhaustive list of factors that vary in the real-world, but our empirical analysis shows that \benchname\ factors do affect the SoTA robot manipulation models, and hence are important to study. While it is challenging to breakdown real-world into an exhaustive systematic enumeration of factors, \benchname\ is one of the first attempt towards increasing real-world task robustness for robotic manipulation. We included more discussion on this in the supplementary material.

[\rtwo{}] \textbf{Consistency on models' action space: } We use a consistent action prediction space for all models for fairer comparison. Recent works \cite{shi2023waypoint} indicate that keypoint or waypoint based action prediction performs better than raw action prediction as it poses an easier learning problem.

[\rtwo{}] \textbf{Similar conclusions as previous works: } We studied the related work and found that a large part of our conclusions are both orthogonal and supplementary to prior work. To summarize the conclusion of related work (FactorWorld) and \benchname,

FactorWorld: Concludes consistency across real-world and sim evaluations, mentioning background, distractors, and lighting are easier while table texture and camera position are harder to generalize to, for image/2D input based models (CLIP, R3M, RT1). Additionally, they conclude that factors do not have compounding effect on generalization. Finally, they study effects data augmentation methods and out-of-domain pre-training data that could improve generalization. 

\benchname: Our results mainly focus on the question: “which perturbation factors affect which class of models”. Our results are partially consistent with FactorWorld for 2D input based models: most affecting factors are color-related and camera pose, while least affecting is Distractors. However, due to inherent hardness of RLBench tasks wrt to MetaWorld tasks, 2D models are not able to learn these tasks well. We additionally report insights for 3D model performance and comparison with 2D models: most affecting factors are color-related and distractors, while least affecting is camera pose. We additionally report an ablation with all perturbation as proxy for an extreme case of factor compounding, which is results in 28.1\% lower in success rates wrt no perturbations. This result is contradictory with prior work. We finally report a comprehensive real-world and simulation alignment analysis, with the same model (PerAct) and simulation tasks reproduced in the real-world. Prior work performs this analysis with RT-1 model on pick tasks in real-world and R3M model on MetaWorld tasks in simulation. From reviewer feedback, we have also included physical perturbation, mass and friction, which are supplementary to prior work. We agree with reviewers that the conclusions are not surprising and rather intuitive, however, we believe that establishing these intuitions empirically and reproducibility have been missing from robotics community and were important to study concretely at this point when the field is ready for real-world robustness measurements.

[\rtwo{}] \textbf{Insights into the difference between pre-trained models and those trained from scratch:}
Our baselines include pretraining on 2D learning models and training from scratch for 3D learning models. These models are architecturally quite different, therefore, it is not an adequately comparable scenario for drawing any conclusions. We hope that future submissions to \benchname\ will be able to bring more light to this discussion.

% \subsection{Reviewer fLen}
% \textbf{Physical properties perturbation:} We concur with the reviewer's assertion on the necessity of benchmarking a model's generalization across physical properties. However, we emphasize that the impact of such perturbations is task-specific. In many quasi-static tasks, changes in physical properties—such as mass, friction, and inertia—do not significantly influence outcomes. Conversely, tasks involving dynamic motion \cite{memmel2023asid}, such as a ball's trajectory after being struck by a hockey stick, are notably affected by these variations. Our benchmarks support a wide range of manipulation policies to enable comprehensive evaluation. Hence to accommodate to this, we have incorporated mass and friction perturbations in our revised work, as detailed in Section \ref{subsec:mass}.




